Learning Structure Aware Deep Spectral Embedding

Spectral Embedding (SE) has often been used to map data points from non-linear manifolds to linear subspaces for the purpose of classification and clustering. Despite significant advantages, the subspace structure of data in the original space is not preserved in the embedding space. To address this issue subspace clustering has been proposed by replacing the SE graph affinity with a self-expression matrix. It works well if the data lies in a union of linear subspaces however, the performance may degrade in real-world applications where data often spans non-linear manifolds. To address this problem we propose a novel structure-aware deep spectral embedding by combining a spectral embedding loss and a structure preservation loss. To this end, a deep neural network architecture is proposed that simultaneously encodes both types of information and aims to generate structure-aware spectral embedding. The subspace structure of the input data is encoded by using attention-based self-expression learning. The proposed algorithm is evaluated on six publicly available real-world datasets. The results demonstrate the excellent clustering performance of the proposed algorithm compared to the existing state-of-the-art methods. The proposed algorithm has also exhibited better generalization to unseen data points and it is scalable to larger datasets without requiring significant computational resources.

==> egbib_bib <==
@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})



@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})

@inproceedings{saha2013sparse,
  title={Sparse subspace clustering via group sparse coding},
  author={Saha, Budhaditya and Pham, Duc Son and Phung, Dinh and Venkatesh, Svetha},
  booktitle={Proceedings of the 2013 SIAM International Conference on Data Mining},
  pages={130--138},
  year={2013},
  organization={SIAM}
}

@InProceedings{Ho04,
  author       = "Ho, J. and Yang, M. H. and Lim, J. and Lee, K. C. and Kriegman, D.",
  title        = "Clustering appearances of objects under varying illumination conditions",
  booktitle    = "Proc. CVPR",
  year         = "2003",
  pages        = "11--18",
}


@article{Kanatani06,
author = {Kanatani, K. I.},
title = {Motion segmentation by subspace separation and model selection},
booktitle = {Proc. ICCV},
volume = 2,
number = 8,
pages = {586--591}, 
year = 2001
}

@InProceedings{Rao09,
  author       = "Rao, S. R. and Tron, R. and Ma, Y.",
  title        = "Motion segmentation via robust subspace separation in the presence of outlying, incomplete, or corrupted trajectories",
  booktitle    = "Proc. CVPR",
  year         = "2008",
  pages        = "1--8",
}

@InProceedings{ Ji10,
  author       = "Ji, P. and  Zhang, T. and Li, H. and Salzmann, M. and Reid, I.",
  title        = "Deep subspace clustering networks",
  booktitle    = "Proc. NIPS",
  year         = "2017"
}

@InProceedings{ Yang11,
  author       = "Yang, J. and Parikh, D. and Batra, D.",
  title        = "Joint unsupervised learning of deep representations and image clusters",
  booktitle    = "Proc. CVPR",
  year         = "2016",
  pages        = "5147--5156",
}

@InProceedings{ Lu12,
  author       = "Lu, C. Y. and Min, H. and Zhao, Z. Q. and Zhu, L. and Huang, D. S. and Yan, S.",
  title        = "Robust and efficient subspace segmentation via least squares regression",
  booktitle    = "Proc. ECCV",
  year         = "2012",
  pages        = "347--360",
}


@article{Xiao13,
author = {Xiao, S. and  Tan, M. and Xu, D. and  Dong, Z. Y.},
title = {Robust kernel low-rank representation},
journal = {IEEE T NEUR NET LEAR},
volume = 27,
number = 11,
pages = {2268--2281}, 
year = 2016
}


@article{Liu14,
author = {Liu, G. and  Lin, Z. and Yan, S. and  Sun, J. and Yu, Y. and  Ma, Y.},
title = {Robust recovery of subspace structures by low-rank representation},
journal = {IEEE NLM},
volume = 35,
number = 1,
pages = {171--184}, 
year = 2013
}

@InProceedings{ Hu15,
  author       = "Hu, H. and Lin, Z. and Feng, J. and Zhou, J.",
  title        = "Smooth representation clustering",
  booktitle    = "Proc. CVPR",
  year         = "2014",
  pages        = "3834--3841",
}

@inproceedings{you2016oracle,
  title={Oracle based active set algorithm for scalable elastic net subspace clustering},
  author={You, Chong and Li, Chun-Guang and Robinson, Daniel P and Vidal, Ren{\'e}},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3928--3937},
  year={2016}
}

@article{Gao16,
author = {Gao, S. and  Tsang, I. W. H. and Chia, L. T.},
title = {Laplacian sparse coding, hypergraph laplacian sparse coding, and applications},
journal = {IEEE NLM},
volume = 35,
number = 1,
pages = {92--104}, 
year = 2013
}

@article{Elhamifar17,
  author={E. {Elhamifar} and R. {Vidal}},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={Sparse Subspace Clustering: Algorithm, Theory, and Applications}, 
  year={2013},}

@InProceedings{ Yang18,
  author       = "Yang, A. Y. and Sastry, S. S. and Ganesh, A. and Ma, Y.",
  title        = "Fast ℓ 1-minimization algorithms and an application in robust face recognition: A review",
  booktitle    = "Proc. ICIP",
  year         = "2010",
  pages        = "1849--1852",
}

@InProceedings{ Xiao19,
  author       = "Xiao, S. and  Li, W. and Xu, D. and Tao, D.",
  title        = "FaLRR: A fast low rank representation solver",
  booktitle    = "Proc. CVPR",
  year         = "2015",
  pages        = "4612--4620",
}

@article{Hinton20,
author = {Hinton, G. E. and Salakhutdinov, R. R.},
title = {Reducing the dimensionality of data with neural networks},
journal = {science},
volume = 313,
number = 5786,
pages = {504--507}, 
year = 2006
}

@article{Roweis21,
author = {Roweis, S. T. and Saul, L. K.},
title = {Nonlinear dimensionality reduction by locally linear embedding},
journal = {science},
volume = 290,
number = 5500,
pages = {2323--2326}, 
year = 2000
}

@article{Vidal22,
author = {Vidal, R. and Favaro, P.},
title = {Low rank subspace clustering},
journal = {Pattern Recognition Letters},
volume = 43,
number = 5500,
pages = {47--61}, 
year = 2014
}

@article{Peng23,
author = {Peng, X. and Feng, J. and Xiao, S. and Yau, W. Y. and Zhou, J. T. and Yang, S.},
title = {Structured autoencoders for subspace clustering},
journal = {IEEE Transactions on Image Processing},
volume = 27,
number = 10,
pages = {5076--5086}, 
year = 2018
}

@InProceedings{Patel24,
  author       = "Patel, V. M. and  Vidal, R.",
  title        = "Kernel sparse subspace clustering",
  booktitle    = "Proc. ICIP",
  year         = "2014",
  pages        = "2849--2853",
}

@InProceedings{Patel25,
  author       = "Patel, V. M. and Van Nguyen, H. and Vidal, R.",
  title        = "Latent space sparse subspace clustering",
  booktitle    = "Proc. ICCV",
  year         = "2013",
  pages        = "225--232",
}

@InProceedings{Tian26,
  author       = "Tian, F. and Gao, B. and Cui, Q. and Chen, E. and Liu, T. Y.",
  title        = "Learning deep representations for graph clustering",
  booktitle    = "Proc. 28th AAAI",
  year         = "2014",
  pages        = "1293--1299",
}

@article{Hu12,
author = {Hu, R. and Fan, L. and Liu, L.},
title = {Co‐segmentation of 3d shapes via subspace clustering},
journal = {Computer graphics forum},
volume = 31,
number = 5,
pages = {1703--1713}, 
year = 2012
}

@article{wu2013unsupervised,
  title={Unsupervised co-segmentation of 3D shapes via affinity aggregation spectral clustering},
  author={Wu, Zizhao and Wang, Yunhai and Shou, Ruyang and Chen, Baoquan and Liu, Xinguo},
  journal={Computers \& Graphics},
  volume={37},
  number={6},
  pages={628--637},
  year={2013},
  publisher={Elsevier}
}


@article{Aldroubi12,
author = {Aldroubi, A. and Sekmen, A.},
title = {Nearness to local subspace algorithm for subspace and motion segmentation},
journal = {IEEE Signal PROC LET},
volume = 19,
number = 10,
pages = {704--707}, 
year = 2012
}

@inproceedings{ng2002,
  author={Ng, A. Y. and Jordan, M. I. and Weiss, Y.},
  title={On spectral clustering: Analysis and an algorithm},
  booktitle={Advances in neural information processing systems},
  pages={849--856},
  year={2002}
}

@inproceedings{ester30,
  title={A density-based algorithm for discovering clusters in large spatial databases with noise.},
  author={Ester, M. and Kriegel, H.P. and Sander, J. and Xu, X.},
  booktitle={Kdd},
  volume={96},
  number={34},
  pages={226--231},
  year={1996}
}

@article{cheng31,
  title={Mean shift, mode seeking, and clustering},
  author={Cheng, Y.},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={17},
  number={8},
  pages={790--799},
  year={1995},
  publisher={IEEE}
}

@article{yang2019subspace,
  title={Subspace clustering via good neighbors},
  author={Yang, Jufeng and Liang, Jie and Wang, Kai and Rosin, Paul L and Yang, Ming-Hsuan},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={42},
  number={6},
  pages={1537--1544},
  year={2019},
  publisher={IEEE}
}
@article{kim2016robust,
  title={Robust elastic-net subspace representation},
  author={Kim, Eunwoo and Lee, Minsik and Oh, Songhwai},
  journal={IEEE Transactions on Image Processing},
  volume={25},
  number={9},
  pages={4245--4259},
  year={2016},
  publisher={IEEE}
}

@article{shaham32,
  title={Spectralnet: Spectral clustering using deep neural networks},
  author={Shaham, Uri and Stanton, Kelly and Li, Henry and Nadler, Boaz and Basri, Ronen and Kluger, Yuval},
  journal={ICLR},
  year={2018}
}

@inproceedings{stella2003multiclass,
  title={Multiclass spectral clustering},
  author={Stella, X Yu and Shi, Jianbo},
  booktitle={null},
  pages={313},
  year={2003},
  organization={IEEE}
}

@article{von2007tutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@article{Talia2013,
  title={Clouds for scalable big data analytics},
  author={Talia, D.},
  journal={Computer},
  volume={46},
  number={5},
  pages={98--101},
  year={2013}
}

@inproceedings{zelnik2005,
  title={Self-tuning spectral clustering},
  author={Zelnik-Manor, Lihi and Perona, Pietro},
  booktitle={Advances in neural information processing systems},
  pages={1601--1608},
  year={2005}
}

@inproceedings{Shi2000,
title={Normalized cuts and image segmentation},
author={Shi, J., and Malik, J.},
booktitle={Departmental Papers (CIS), 107},
year={2000}
}

@inproceedings{Peng2013,
title={Scalable sparse subspace clustering},
author={Peng, X., Zhang, L., and Yi, Z.},
booktitle={Proc. CVPR},
pages={430--437},
year={2013}
}

@inproceedings{He2004,
title={Locality preserving projections},
author={He, X., and Niyogi, P.},
booktitle={Proc. NIPS},
pages={153--160},
year={2004}
}

@inproceedings{Liu2010,
title={Large graph construction for scalable semi-supervised learning},
author={Liu, W., He, J., and Chang, S. F.},
booktitle={ICML-10},
pages={679--686},
year={2010}
}

@inproceedings{Khusro2016,
title={Recommender systems: issues, challenges, and research opportunities},
author={Khusro, S., Ali, Z., and Ullah, I.},
booktitle={In Information Science and Applications (ICISA)},
pages={1179--1189},
year={2016},
publisher={Springer}
}

@inproceedings{Li2011,
title={SCENE: a scalable two-stage personalized news recommendation system},
author={Li, L., Wang, D., Li, T., Knox, D., and Padmanabhan, B.},
booktitle={In Proceedings of the 34th international ACM SIGIR conference on Research and development in Information Retrieval},
pages={125--134},
year={2011}
}

@article{Lu2019,
  title={Subspace clustering by block diagonal representation},
  author={Lu, C., Feng, J., Lin, Z., Mei, T., and Yan, S.},
  journal={IEEE transactions on pattern analysis and machine intelligence (PAMI)},
  volume={41},
  number={2},
  pages={487--501},
  year={2019}
}

@article{Peng2016,
  title={Connections between nuclear-norm and frobenius-norm-based representations},
  author={Peng, X., Lu, C., Yi, Z., and Tang, H.},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={1},
  pages={218--224},
  year={2016}
}

@article{chen2018subspace,
  title={Subspace clustering using a low-rank constrained autoencoder},
  author={Chen, Yuanyuan and Zhang, Lei and Yi, Zhang},
  journal={Information Sciences},
  volume={424},
  pages={27--38},
  year={2018},
  publisher={Elsevier}
}

@article{yang2019subspace,
  title={Subspace Clustering via Good Neighbors},
  author={Yang, Jufeng and Liang, Jie and Wang, Kai and Rosin, Paul and Yang, Ming-Hsuan},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  year={2019},
  publisher={IEEE}
}

@inproceedings{tian2019subspace,
  title={Subspace Clustering Based on Self-organizing Map},
  author={Tian, Jin and Gu, Mengyi},
  booktitle={Proceeding of the 24th International Conference on Industrial Engineering and Engineering Management 2018},
  pages={151--159},
  year={2019},
  organization={Springer}
}

@article{zhang2018generalized,
  title={Generalized latent multi-view subspace clustering},
  author={Zhang, Changqing and Fu, Huazhu and Hu, Qinghua and Cao, Xiaochun and Xie, Yuan and Tao, Dacheng and Xu, Dong},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  year={2018},
  publisher={IEEE}
}

@article{abavisani2018deep,
  title={Deep Multimodal Subspace Clustering Networks},
  author={Abavisani, Mahdi and Patel, Vishal M},
  journal={IEEE Journal of Selected Topics in Signal Processing},
  volume={12},
  number={6},
  pages={1601--1614},
  year={2018},
  publisher={IEEE}
}

@article{wang2018beyond,
  title={Beyond low-rank representations: Orthogonal clustering basis reconstruction with optimized graph structure for multi-view spectral clustering},
  author={Wang, Yang and Wu, Lin},
  journal={Neural Networks},
  volume={103},
  pages={1--8},
  year={2018},
  publisher={Elsevier}
}

@article{tang2018learning,
  title={Learning Joint Affinity Graph for Multi-view Subspace Clustering},
  author={Tang, Chang and Zhu, Xinzhong and Liu, Xinwang and Li, Miaomiao and Wang, Pichao and Zhang, Changqing and Wang, Lizhe},
  journal={IEEE Transactions on Multimedia},
  year={2018},
  publisher={IEEE}
}

@article{yang2019deep,
author = {Yang, Xu and Deng, Cheng and Zheng, Feng and Yan, Junchi and Liu, Wei},
title = {Deep Spectral Clustering Using Dual Autoencoder Network},
booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}


@inproceedings{zhou2018iterative,
  title={Iterative Deep Subspace Clustering},
  author={Zhou, Lei and Wang, Shuai and Bai, Xiao and Zhou, Jun and Hancock, Edwin},
  booktitle={Joint IAPR International Workshops on Statistical Techniques in Pattern Recognition (SPR) and Structural and Syntactic Pattern Recognition (SSPR)},
  pages={42--51},
  year={2018},
  organization={Springer}
}

@article{yang2019three,
  title={Three-Stage Subspace Clustering Framework with Graph-Based Transformation and Optimization},
  author={Yang, Shuai and Zhu, Wenqi and Zhu, Yuesheng},
  journal={arXiv preprint arXiv:1905.01145},
  year={2019}
}

@article{zhang2019robust,
  title={Robust low-rank kernel multi-view subspace clustering based on the Schatten p-norm and correntropy},
  author={Zhang, Xiaoqian and Sun, Huaijiang and Liu, Zhigui and Ren, Zhenwen and Cui, Qiongjie and Li, Yanmeng},
  journal={Information Sciences},
  volume={477},
  pages={430--447},
  year={2019},
  publisher={Elsevier}
}

@article{chen2019locality,
  title={Locality-constrained least squares regression for subspace clustering},
  author={Chen, Yuanyuan and Yi, Zhang},
  journal={Knowledge-Based Systems},
  volume={163},
  pages={51--56},
  year={2019},
  publisher={Elsevier}
}

@article{bian2019joint,
  title={Joint Learning of Spectral Clustering Structure and Fuzzy Similarity Matrix of Data},
  author={Bian, Zekang and Ishibuchi, Hisao and Wang, Shitong},
  journal={IEEE Transactions on Fuzzy Systems},
  volume={27},
  number={1},
  pages={31--44},
  year={2019},
  publisher={IEEE}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick and others},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Taipei, Taiwan}
}

@article{basri2003lambertian,
  title={Lambertian reflectance and linear subspaces},
  author={Basri, Ronen and Jacobs, David W},
  journal={IEEE Transactions on Pattern Analysis \& Machine Intelligence},
  number={2},
  pages={218--233},
  year={2003},
  publisher={IEEE}
}

@article{hastie1998metrics,
  title={Metrics and models for handwritten character recognition},
  author={Hastie, Trevor and Simard, Patrice Y},
  journal={Statistical Science},
  pages={54--65},
  year={1998},
  publisher={JSTOR}
}

@article{lee2005acquiring,
  title={Acquiring linear subspaces for face recognition under variable lighting},
  author={Lee, Kuang-Chih and Ho, Jeffrey and Kriegman, David J},
  journal={IEEE Transactions on Pattern Analysis \& Machine Intelligence},
  number={5},
  pages={684--698},
  year={2005},
  publisher={IEEE}
}

@article{lewitus2019characterizing,
  title={Characterizing and comparing phylogenetic trait data from their normalized Laplacian spectrum},
  author={Lewitus, Eric and Aristide, Leandro and Morlon, Helene},
  journal={bioRxiv},
  pages={654087},
  year={2019},
  publisher={Cold Spring Harbor Laboratory}
}

@article{shastri2019vector,
  title={Vector Quantized Spectral Clustering Applied to Whole Genome Sequences of Plants},
  author={Shastri, Aditya A and Ahuja, Kapil and Ratnaparkhe, Milind B and Shah, Aditya and Gagrani, Aishwary and Lal, Anant},
  journal={Evolutionary Bioinformatics},
  volume={15},
  pages={1176934319836997},
  year={2019},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{shastri2018vector,
  title={Vector Quantized Spectral Clustering applied to Soybean Whole Genome Sequences},
  author={Shastri, Aditya A and Ahuja, Kapil and Ratnaparkhe, Milind B and Shah, Aditya and Gagrani, Aishwary and Lal, Anant},
  journal={arXiv preprint arXiv:1810.00398},
  year={2018}
}

@inproceedings{coates2011analysis,
  title={An analysis of single-layer networks in unsupervised feature learning},
  author={Coates, Adam and Ng, Andrew and Lee, Honglak},
  booktitle={Proceedings of the fourteenth international conference on artificial intelligence and statistics},
  pages={215--223},
  year={2011}
}

@article{yin2018ensemble,
  title={Ensemble biclustering gene expression data based on the spectral clustering},
  author={Yin, Lu and Liu, Yongguo},
  journal={Neural Computing and Applications},
  volume={30},
  number={8},
  pages={2403--2416},
  year={2018},
  publisher={Springer}
}

@article{shen2017distance,
  title={A distance-based spectral clustering approach with applications to network community detection},
  author={Shen, Gang and Ye, Dongmei},
  journal={Journal of Industrial Information Integration},
  volume={6},
  pages={22--32},
  year={2017},
  publisher={Elsevier}
}

@article{li2018local,
  title={Local spectral clustering for overlapping community detection},
  author={Li, Yixuan and He, Kun and Kloster, Kyle and Bindel, David and Hopcroft, John},
  journal={ACM Transactions on Knowledge Discovery from Data (TKDD)},
  volume={12},
  number={2},
  pages={17},
  year={2018},
  publisher={ACM}
}

@article{li2018overlap,
  title={Overlap community detection using spectral algorithm based on node convergence degree},
  author={Li, Weimin and Jiang, Shu and Jin, Qun},
  journal={Future Generation Computer Systems},
  volume={79},
  pages={408--416},
  year={2018},
  publisher={Elsevier}
}

@article{liu2018global,
  title={Global spectral clustering in dynamic networks},
  author={Liu, Fuchen and Choi, David and Xie, Lu and Roeder, Kathryn},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={5},
  pages={927--932},
  year={2018},
  publisher={National Acad Sciences}
}

@inproceedings{wasito2018iterative,
  title={Iterative Scaling Fuzzy Additive Spectral Clustering (is-FADDIS) Algorithm for Subtypes Cancer Identification using Gene Expression Data},
  author={Wasito, Ito and Fathurahman, Muhamad and Veritawati, Ionia and Budi, Indra and Sari, Betha Nurina},
  booktitle={Proceedings of the 2018 8th International Conference on Bioscience, Biochemistry and Bioinformatics},
  pages={6--9},
  year={2018},
  organization={ACM}
}

@article{banerjee2019spectral,
  title={Spectral clustering via sparse graph structure learning with application to proteomic signaling networks in cancer},
  author={Banerjee, Sayantan and Akbani, Rehan and Baladandayuthapani, Veerabhadran},
  journal={Computational Statistics \& Data Analysis},
  volume={132},
  pages={46--69},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{you2016scalable,
  title={Scalable sparse subspace clustering by orthogonal matching pursuit},
  author={You, Chong and Robinson, Daniel and Vidal, Ren{\'e}},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3918--3927},
  year={2016}
}

@article{tung2010enabling,
  title={Enabling scalable spectral clustering for image segmentation},
  author={Tung, Frederick and Wong, Alexander and Clausi, David A},
  journal={Pattern Recognition},
  volume={43},
  number={12},
  pages={4069--4076},
  year={2010},
  publisher={Elsevier}
}

@article{cai2014large,
  title={Large scale spectral clustering via landmark-based sparse representation},
  author={Cai, Deng and Chen, Xinlei},
  journal={IEEE transactions on cybernetics},
  volume={45},
  number={8},
  pages={1669--1680},
  year={2014},
  publisher={IEEE}
}

@inproceedings{song2008parallel,
  title={Parallel spectral clustering},
  author={Song, Yangqiu and Chen, Wen-Yen and Bai, Hongjie and Lin, Chih-Jen and Chang, Edward Y},
  booktitle={Joint European conference on machine learning and knowledge discovery in databases},
  pages={374--389},
  year={2008},
  organization={Springer}
}


@article{chen2010parallel,
  title={Parallel spectral clustering in distributed systems},
  author={Chen, Wen-Yen and Song, Yangqiu and Bai, Hongjie and Lin, Chih-Jen and Chang, Edward Y},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={33},
  number={3},
  pages={568--586},
  year={2010},
  publisher={IEEE}
}

@article{falkner2008spectral,
  title={A spectral clustering approach to MS/MS identification of post-translational modifications},
  author={Falkner, Jayson A and Falkner, Jarret W and Yocum, Anastasia K and Andrews, Philip C},
  journal={Journal of proteome research},
  volume={7},
  number={11},
  pages={4614--4622},
  year={2008},
  publisher={ACS Publications}
}

@article{griss2016spectral,
  title={Spectral library searching in proteomics},
  author={Griss, Johannes},
  journal={Proteomics},
  volume={16},
  number={5},
  pages={729--740},
  year={2016},
  publisher={Wiley Online Library}
}

@article{liu2008analysis,
  title={Analysis of correlated mutations in HIV-1 protease using spectral clustering},
  author={Liu, Ying and Eyal, Eran and Bahar, Ivet},
  journal={Bioinformatics},
  volume={24},
  number={10},
  pages={1243--1250},
  year={2008},
  publisher={Oxford University Press}
}

@article{paccanaro2006spectral,
  title={Spectral clustering of protein sequences},
  author={Paccanaro, Alberto and Casbon, James A and Saqi, Mansoor AS},
  journal={Nucleic acids research},
  volume={34},
  number={5},
  pages={1571--1580},
  year={2006},
  publisher={Oxford University Press}
}

@article{kluger2003spectral,
  title={Spectral biclustering of microarray data: coclustering genes and conditions},
  author={Kluger, Yuval and Basri, Ronen and Chang, Joseph T and Gerstein, Mark},
  journal={Genome research},
  volume={13},
  number={4},
  pages={703--716},
  year={2003},
  publisher={Cold Spring Harbor Lab}
}

@article{chen2009spectral,
  title={Spectral curvature clustering (SCC)},
  author={Chen, Guangliang and Lerman, Gilad},
  journal={International Journal of Computer Vision},
  volume={81},
  number={3},
  pages={317--330},
  year={2009},
  publisher={Springer}
}

@inproceedings{you2016oracle,
  title={Oracle based active set algorithm for scalable elastic net subspace clustering},
  author={You, Chong and Li, Chun-Guang and Robinson, Daniel P and Vidal, Ren{\'e}},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={3928--3937},
  year={2016}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{you2018scalable,
  title={Scalable exemplar-based subspace clustering on class-imbalanced data},
  author={You, Chong and Li, Chi and Robinson, Daniel P and Vidal, Ren{\'e}},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={67--83},
  year={2018}
}


@inproceedings{shen2016online,
  title={Online low-rank subspace clustering by basis dictionary pursuit},
  author={Shen, Jie and Li, Ping and Xu, Huan},
  booktitle={International Conference on Machine Learning},
  pages={622--631},
  year={2016}
}

@article{abdolali2019scalable,
  title={Scalable and robust sparse subspace clustering using randomized clustering and multilayer graphs},
  author={Abdolali, Maryam and Gillis, Nicolas and Rahmati, Mohammad},
  journal={Signal Processing},
  volume={163},
  pages={166--180},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{you2018scalable,
  title={Scalable exemplar-based subspace clustering on class-imbalanced data},
  author={You, Chong and Li, Chi and Robinson, Daniel P and Vidal, Ren{\'e}},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={67--83},
  year={2018}
}

@inproceedings{chen2020stochastic,
  title={Stochastic Sparse Subspace Clustering},
  author={Chen, Ying and Li, Chun-Guang and You, Chong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4155--4164},
  year={2020}
}

@article{bruna2013invariant,
  title={Invariant scattering convolution networks},
  author={Bruna, Joan and Mallat, St{\'e}phane},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={35},
  number={8},
  pages={1872--1886},
  year={2013},
  publisher={IEEE}
}

@inproceedings{kheirandishfard2020deep,
  title={Deep Low-Rank Subspace Clustering},
  author={Kheirandishfard, Mohsen and Zohrizadeh, Fariba and Kamangar, Farhad},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops},
  pages={864--865},
  year={2020}
}

@article{georghiades2001few,
  title={From few to many: Illumination cone models for face recognition under variable lighting and pose},
  author={Georghiades, Athinodoros S. and Belhumeur, Peter N. and Kriegman, David J.},
  journal={IEEE Trans on Pattern Analysis and Mach. Int.},
  volume={23},
  number={6},
  pages={643--660},
  year={2001},
  publisher={IEEE}
}

@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Citeseer}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}

@inproceedings{tian2014learning,
  title={Learning deep representations for graph clustering.},
  author={Tian, Fei and Gao, Bin and Cui, Qing and Chen, Enhong and Liu, Tie-Yan},
  booktitle={Aaai},
  volume={14},
  pages={1293--1299},
  year={2014},
  organization={Citeseer}
}

@inproceedings{seo2019deep,
  title={Deep Closed-Form Subspace Clustering},
  author={Seo, Junghoon and Koo, Jamyoung and Jeon, Taegyun},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision Workshops},
  pages={0--0},
  year={2019}
}

@inproceedings{guo2017improved,
  title={Improved deep embedded clustering with local structure preservation},
  author={Guo, Xifeng and Gao, Long and Liu, Xinwang and Yin, Jianping},
  booktitle={IJCAI},
  pages={1753--1759},
  year={2017}
}

@inproceedings{xie2016unsupervised,
  title={Unsupervised deep embedding for clustering analysis},
  author={Xie, Junyuan and Girshick, Ross and Farhadi, Ali},
  booktitle={International conference on machine learning},
  pages={478--487},
  year={2016}
}

@inproceedings{zhou2018deep,
  title={Deep adversarial subspace clustering},
  author={Zhou, Pan and Hou, Yunqing and Feng, Jiashi},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={1596--1604},
  year={2018}
}

@article{jiang2016variational,
  title={Variational deep embedding: An unsupervised and generative approach to clustering},
  author={Jiang, Zhuxi and Zheng, Yin and Tan, Huachun and Tang, Bangsheng and Zhou, Hanning},
  journal={arXiv preprint arXiv:1611.05148},
  year={2016}
}

@article{yu2020gan,
  title={GAN-based enhanced deep subspace clustering networks},
  author={Yu, Zhiwen and Zhang, Zhongfan and Cao, Wenming and Liu, Cheng and Chen, Junlong Philip and San Wong, Hau},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2020},
  publisher={IEEE}
}

@article{Zeiler2012ADADELTAAA,
  title={ADADELTA: An Adaptive Learning Rate Method},
  author={Matthew D. Zeiler},
  journal={ArXiv},
  year={2012},
  volume={abs/1212.5701}
}

@inproceedings{zhang2019self,
  title={Self-supervised convolutional subspace clustering network},
  author={Zhang, Junjian and Li, Chun-Guang and You, Chong and Qi, Xianbiao and Zhang, Honggang and Guo, Jun and Lin, Zhouchen},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={5473--5482},
  year={2019}
}

@article{abavisani2020deep,
  title={Deep Subspace Clustering with Data Augmentation},
  author={Abavisani, Mahdi and Naghizadeh, Alireza and Metaxas, Dimitris and Patel, Vishal},
  journal={Adv. in Neural Info. Processing Systems},
  volume={33},
  year={2020}
}

@inproceedings{peng2017cascade,
  title={Cascade subspace clustering},
  author={Peng, Xi and Feng, Jiashi and Lu, Jiwen and Yau, Wei-Yun and Yi, Zhang},
  booktitle={Thirty-First AAAI conference on artificial intelligence},
  year={2017}
}

@article{busch2020learning,
  title={Learning Self-Expression Metrics for Scalable and Inductive Subspace Clustering},
  author={Busch, Julian and Faerman, Evgeniy and Schubert, Matthias and Seidl, Thomas},
  journal={arXiv preprint arXiv:2009.12875},
  year={2020}
}

@inproceedings{zhang2018scalable,
  title={Scalable deep k-subspace clustering},
  author={Zhang, Tong and Ji, Pan and Harandi, Mehrtash and Hartley, Richard and Reid, Ian},
  booktitle={Asian Conference on Computer Vision},
  pages={466--481},
  year={2018},
  organization={Springer}
}

@article{xia2017human,
  title={Human motion segmentation via robust kernel sparse subspace clustering},
  author={Xia, Guiyu and Sun, Huaijiang and Feng, Lei and Zhang, Guoqing and Liu, Yazhou},
  journal={IEEE Transactions on Image Processing},
  volume={27},
  number={1},
  pages={135--150},
  year={2017},
  publisher={IEEE}
}

@article{li2017structured,
  title={Structured sparse subspace clustering: A joint affinity learning and subspace clustering framework},
  author={Li, Chun-Guang and You, Chong and Vidal, Ren{\'e}},
  journal={IEEE Transactions on Image Processing},
  volume={26},
  number={6},
  pages={2988--3001},
  year={2017},
  publisher={IEEE}
}

@article{liu2019robust,
  title={Robust subspace clustering with compressed data},
  author={Liu, Guangcan and Zhang, Zhao and Liu, Qingshan and Xiong, Hongkai},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={10},
  pages={5161--5170},
  year={2019},
  publisher={IEEE}
}

@article{he2015robust,
  title={Robust subspace clustering with complex noise},
  author={He, Ran and Zhang, Yingya and Sun, Zhenan and Yin, Qiyue},
  journal={IEEE Transactions on Image Processing},
  volume={24},
  number={11},
  pages={4001--4013},
  year={2015},
  publisher={IEEE}
}

@article{lv2021pseudo,
  title={Pseudo-supervised deep subspace clustering},
  author={Lv, Juncheng and Kang, Zhao and Lu, Xiao and Xu, Zenglin},
  journal={IEEE Transactions on Image Processing},
  volume={30},
  pages={5252--5263},
  year={2021},
  publisher={IEEE}
}

@article{yang2019split,
  title={Split multiplicative multi-view subspace clustering},
  author={Yang, Zhiyong and Xu, Qianqian and Zhang, Weigang and Cao, Xiaochun and Huang, Qingming},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={10},
  pages={5147--5160},
  year={2019},
  publisher={IEEE}
}

@article{yin2018subspace,
  title={Subspace clustering via learning an adaptive low-rank graph},
  author={Yin, Ming and Xie, Shengli and Wu, Zongze and Zhang, Yun and Gao, Junbin},
  journal={IEEE Transactions on Image Processing},
  volume={27},
  number={8},
  pages={3716--3728},
  year={2018},
  publisher={IEEE}
}


@inproceedings{sekmen2013subspace,
  title={Subspace and motion segmentation via local subspace estimation},
  author={Sekmen, Ali and Aldroubi, Akram},
  booktitle={2013 IEEE Workshop on Robot Vision (WORV)},
  pages={27--33},
  year={2013},
  organization={IEEE}
}

@article{wang2014video,
  title={Video object co-segmentation via subspace clustering and quadratic pseudo-boolean optimization in an MRF framework},
  author={Wang, Chuan and Guo, Yanwen and Zhu, Jie and Wang, Linbo and Wang, Wenping},
  journal={IEEE Transactions on Multimedia},
  volume={16},
  number={4},
  pages={903--916},
  year={2014},
  publisher={IEEE}
}

@article{nene1996columbia,
  title={Columbia university image library (coil-20)},
  author={Nene, SA and Nayar, SK and Murase, H},
  journal={Technical Report CUCS-005-96},
  year={1996}
}

@inproceedings{peng2016deep,
  title={Deep subspace clustering with sparsity prior},
  author={Peng, Xi and Xiao, Shijie and Feng, Jiashi and Yau, Wei-Yun and Yi, Zhang},
  booktitle={IJCAI},
  pages={1925--1931},
  year={2016}
}

@article{li2018discriminatively,
  title={Discriminatively boosted image clustering with fully convolutional auto-encoders},
  author={Li, Fengfu and Qiao, Hong and Zhang, Bo},
  journal={Pattern Recognition},
  volume={83},
  pages={161--173},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{zhang2012graph,
  title={Graph degree linkage: Agglomerative clustering on a directed graph},
  author={Zhang, Wei and Wang, Xiaogang and Zhao, Deli and Tang, Xiaoou},
  booktitle={European Conference on Computer Vision},
  pages={428--441},
  year={2012},
  organization={Springer}
}

@article{zhu2018low,
  title={Low-rank sparse subspace for spectral clustering},
  author={Zhu, Xiaofeng and Zhang, Shichao and Li, Yonggang and Zhang, Jilian and Yang, Lifeng and Fang, Yue},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={31},
  number={8},
  pages={1532--1543},
  year={2018},
  publisher={IEEE}
}

@article{li2018rank,
  title={Rank-constrained spectral clustering with flexible embedding},
  author={Li, Zhihui and Nie, Feiping and Chang, Xiaojun and Nie, Liqiang and Zhang, Huaxiang and Yang, Yi},
  journal={IEEE transactions on neural networks and learning systems},
  volume={29},
  number={12},
  pages={6073--6082},
  year={2018},
  publisher={IEEE}
}

@inproceedings{kheirandishfard2020multi,
  title={Multi-level representation learning for deep subspace clustering},
  author={Kheirandishfard, Mohsen and Zohrizadeh, Fariba and Kamangar, Farhad},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={2039--2048},
  year={2020}
}

@article{krizhevsky2009learning,
  title={Learning multiple layers of features from tiny images},
  author={Krizhevsky, Alex and Hinton, Geoffrey and others},
  year={2009},
  publisher={Toronto, ON, Canada}
}

@inproceedings{yang2016joint,
  title={Joint unsupervised learning of deep representations and image clusters},
  author={Yang, Jianwei and Parikh, Devi and Batra, Dhruv},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={5147--5156},
  year={2016}
}

@inproceedings{xie2016unsupervised,
  title={Unsupervised deep embedding for clustering analysis},
  author={Xie, Junyuan and Girshick, Ross and Farhadi, Ali},
  booktitle={International conference on machine learning},
  pages={478--487},
  year={2016},
  organization={PMLR}
}

@article{chang2019deep,
  title={Deep discriminative clustering analysis},
  author={Chang, Jianlong and Guo, Yiwen and Wang, Lingfeng and Meng, Gaofeng and Xiang, Shiming and Pan, Chunhong},
  journal={arXiv preprint arXiv:1905.01681},
  year={2019}
}

@article{li2022twin,
  title={Twin contrastive learning for online clustering},
  author={Li, Yunfan and Yang, Mouxing and Peng, Dezhong and Li, Taihao and Huang, Jiantao and Peng, Xi},
  journal={International Journal of Computer Vision},
  volume={130},
  number={9},
  pages={2205--2221},
  year={2022},
  publisher={Springer}
}
@article{li2020prototypical,
  title={Prototypical contrastive learning of unsupervised representations},
  author={Li, Junnan and Zhou, Pan and Xiong, Caiming and Hoi, Steven CH},
  journal={arXiv preprint arXiv:2005.04966},
  year={2020}
}

@inproceedings{van2020scan,
  title={Scan: Learning to classify images without labels},
  author={Van Gansbeke, Wouter and Vandenhende, Simon and Georgoulis, Stamatios and Proesmans, Marc and Van Gool, Luc},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part X},
  pages={268--285},
  year={2020},
  organization={Springer}
}
@article{niu2022spice,
  title={Spice: Semantic pseudo-labeling for image clustering},
  author={Niu, Chuang and Shan, Hongming and Wang, Ge},
  journal={IEEE Transactions on Image Processing},
  volume={31},
  pages={7264--7278},
  year={2022},
  publisher={IEEE}
}

@inproceedings{li2021contrastive,
  title={Contrastive clustering},
  author={Li, Yunfan and Hu, Peng and Liu, Zitao and Peng, Dezhong and Zhou, Joey Tianyi and Peng, Xi},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={10},
  pages={8547--8555},
  year={2021}
}

@inproceedings{huang2020deep,
  title={Deep semantic clustering by partition confidence maximisation},
  author={Huang, J and Gong, S and Zhu, X},
  booktitle={Pro.  Conference on Computer Vision and Pattern Recognition},
  year={2020}
}

@inproceedings{wu2019deep,
  title={Deep comprehensive correlation mining for image clustering},
  author={Wu, Jianlong and Long, Keyu and Wang, Fei and Qian, Chen and Li, Cheng and Lin, Zhouchen and Zha, Hongbin},
  booktitle={Proceedings of the IEEE/CVF international conference on computer vision},
  pages={8150--8159},
  year={2019}
}

@inproceedings{ji2019invariant,
  title={Invariant information clustering for unsupervised image classification and segmentation},
  author={Ji, Xu and Henriques, Joao F and Vedaldi, Andrea},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9865--9874},
  year={2019}
}
@inproceedings{chang2017deep,
  title={Deep adaptive image clustering},
  author={Chang, Jianlong and Wang, Lingfeng and Meng, Gaofeng and Xiang, Shiming and Pan, Chunhong},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5879--5887},
  year={2017}
}

@inproceedings{guo2017improved,
  title={Improved deep embedded clustering with local structure preservation.},
  author={Guo, Xifeng and Gao, Long and Liu, Xinwang and Yin, Jianping},
  booktitle={Ijcai},
  pages={1753--1759},
  year={2017}
}

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@article{bengio2006greedy,
  title={Greedy layer-wise training of deep networks},
  author={Bengio, Yoshua and Lamblin, Pascal and Popovici, Dan and Larochelle, Hugo},
  journal={Adv. in Neural Info. Processing Systems},
  volume={19},
  year={2006}
}

@inproceedings{haeusser2019associative,
  title={Associative deep clustering: Training a classification network with no labels},
  author={Haeusser, Philip and Plapp, Johannes and Golkov, Vladimir and Aljalbout, Elie and Cremers, Daniel},
  booktitle={Pattern Recognition: 40th German Conference, Oct. 9-12,},
  pages={18--32},
  year={2019}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}

@inproceedings{zeiler2010deconvolutional,
  title={Deconvolutional networks},
  author={Zeiler, Matthew D and Krishnan, Dilip and Taylor, Graham W and Fergus, Rob},
  booktitle={2010 IEEE Computer Society Conference on computer vision and pattern recognition},
  pages={2528--2535},
  year={2010},
  organization={IEEE}
}

@article{radford2015unsupervised,
  title={Unsupervised representation learning with deep convolutional generative adversarial networks},
  author={Radford, Alec and Metz, Luke and Chintala, Soumith},
  journal={arXiv preprint arXiv:1511.06434},
  year={2015}
}

@article{vincent2010stacked,
  title={Stacked denoising autoencoders: Learning useful representations in a deep network with a local denoising criterion.},
  author={Vincent, Pascal and Larochelle, Hugo and Lajoie, Isabelle and Bengio, Yoshua and Manzagol, Pierre-Antoine and Bottou, L{\'e}on},
  journal={Journal of machine learning research},
  volume={11},
  number={12},
  year={2010}
}


@inproceedings{chang2017deep,
  title={Deep adaptive image clustering},
  author={Chang, Jianlong and Wang, Lingfeng and Meng, Gaofeng and Xiang, Shiming and Pan, Chunhong},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5879--5887},
  year={2017}
}

@inproceedings{li2019reciprocal,
  title={Reciprocal multi-layer subspace learning for multi-view clustering},
  author={Li, Ruihuang and Zhang, Changqing and Fu, Huazhu and Peng, Xi and Zhou, Tianyi and Hu, Qinghua},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={8172--8180},
  year={2019}
}

@article{matsushima2019selective,
  title={Selective sampling-based scalable sparse subspace clustering},
  author={Matsushima, Shin and Brbic, Maria},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  pages={12416--12425},
  year={2019}
}

@article{lv2021pseudo,
  title={Pseudo-supervised deep subspace clustering},
  author={Lv, Juncheng and Kang, Zhao and Lu, Xiao and Xu, Zenglin},
  journal={IEEE Transactions on Image Processing},
  volume={30},
  pages={5252--5263},
  year={2021},
  publisher={IEEE}
}

@article{huang2020deep,
  title={Deep subspace clustering to achieve jointly latent feature extraction and discriminative learning},
  author={Huang, Qinjian and Zhang, Yue and Peng, Hong and Dan, Tingting and Weng, Wanlin and Cai, Hongmin},
  journal={Neurocomputing},
  volume={404},
  pages={340--350},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{zhang2019neural,
  title={Neural collaborative subspace clustering},
  author={Zhang, Tong and Ji, Pan and Harandi, Mehrtash and Huang, Wenbing and Li, Hongdong},
  booktitle={International Conference on Machine Learning},
  pages={7384--7393},
  year={2019},
  organization={PMLR}
}

@article{peng2021maximum,
  title={Maximum entropy subspace clustering network},
  author={Peng, Zhihao and Jia, Yuheng and Liu, Hui and Hou, Junhui and Zhang, Qingfu},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  year={2021},
  publisher={IEEE}
}

@article{kang2020relation,
  title={Relation-guided representation learning},
  author={Kang, Zhao and Lu, Xiao and Liang, Jian and Bai, Kun and Xu, Zenglin},
  journal={Neural Networks},
  volume={131},
  pages={93--102},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{ma2020towards,
  title={Towards clustering-friendly representations: subspace clustering via graph filtering},
  author={Ma, Zhengrui and Kang, Zhao and Luo, Guangchun and Tian, Ling and Chen, Wenyu},
  booktitle={Proceedings of the 28th ACM International Conference on Multimedia},
  pages={3081--3089},
  year={2020}
}

@inproceedings{yang2020residual,
  title={Residual encoder-decoder network for deep subspace clustering},
  author={Yang, Shuai and Zhu, Wenqi and Zhu, Yuesheng},
  booktitle={2020 IEEE International Conference on Image Processing (ICIP)},
  pages={2895--2899},
  year={2020},
  organization={IEEE}
}

@article{li2020autoencoder,
  title={Autoencoder constrained clustering with adaptive neighbors},
  author={Li, Xuelong and Zhang, Rui and Wang, Qi and Zhang, Hongyuan},
  journal={IEEE transactions on neural networks and learning systems},
  volume={32},
  number={1},
  pages={443--449},
  year={2020},
  publisher={IEEE}
}

@article{shi2019multi,
  title={Multi-view subspace clustering analysis for aggregating multiple heterogeneous omics data},
  author={Shi, Qianqian and Hu, Bing and Zeng, Tao and Zhang, Chuanchao},
  journal={Frontiers in genetics},
  pages={744},
  year={2019},
  publisher={Frontiers}
}

@article{wallace2015application,
  title={Application of subspace clustering in dna sequence analysis},
  author={Wallace, Tim and Sekmen, Ali and Wang, Xiaofei},
  journal={Journal of Computational Biology},
  volume={22},
  number={10},
  pages={940--952},
  year={2015},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}

@article{tchagang2014subspace,
  title={Subspace clustering of dna microarray data: Theory, evaluation, and applications},
  author={Tchagang, Alain B and Famili, Fazel and Pan, Youlian},
  journal={International Journal of Computational Models and Algorithms in Medicine (IJCMAM)},
  volume={4},
  number={2},
  pages={1--52},
  year={2014},
  publisher={IGI Global}
}

@inproceedings{ciortan2021optimization,
  title={Optimization algorithm for omic data subspace clustering},
  author={Ciortan, Madalina and Defrance, Matthieu},
  booktitle={The 12th International Conference on Computational Systems-Biology and Bioinformatics},
  pages={69--89},
  year={2021}
}

@article{wang2019generalized,
  title={Generalized gene co-expression analysis via subspace clustering using low-rank representation},
  author={Wang, Tongxin and Zhang, Jie and Huang, Kun},
  journal={BMC bioinformatics},
  volume={20},
  number={7},
  pages={17--27},
  year={2019},
  publisher={BioMed Central}
}

@inproceedings{griffith2009kiwi,
  title={KiWi: A scalable subspace clustering algorithm for gene expression analysis},
  author={Griffith, Obi L and Gao, Byron J and Bilenky, Mikhail and Prychyna, Yuliya and Ester, Martin and Jones, Steven JM},
  booktitle={2009 3rd International Conference on Bioinformatics and Biomedical Engineering},
  pages={1--9},
  year={2009},
  organization={IEEE}
}

@article{peng2021adaptive,
  title={Adaptive Attribute and Structure Subspace Clustering Network},
  author={Peng, Zhihao and Liu, Hui and Jia, Yuheng and Hou, Junhui},
  journal={arXiv preprint arXiv:2109.13742},
  year={2021}
}

@inproceedings{ghasedi2019balanced,
  title={Balanced self-paced learning for generative adversarial clustering network},
  author={Ghasedi, Kamran and Wang, Xiaoqian and Deng, Cheng and Huang, Heng},
  booktitle={Proc. of the  Conference on Computer Vision and Pattern Recognition},
  pages={4391--4400},
  year={2019}
}

@inproceedings{ghasedi2017deep,
  title={Deep clustering via joint convolutional autoencoder embedding and relative entropy minimization},
  author={Ghasedi Dizaji, Kamran and Herandi, Amirhossein and Deng, Cheng and Cai, Weidong and Huang, Heng},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5736--5745},
  year={2017}
}

@article{roweis2000nonlinear,
  title={Nonlinear dimensionality reduction by locally linear embedding},
  author={Roweis, Sam T and Saul, Lawrence K},
  journal={science},
  volume={290},
  number={5500},
  pages={2323--2326},
  year={2000},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{valanarasu2021overcomplete,
  title={Overcomplete deep subspace clustering networks},
  author={Valanarasu, Jeya Maria Jose and Patel, Vishal M},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={746--755},
  year={2021}
}

@article{vielhaben2022sparse,
  title={Sparse subspace clustering for concept discovery (SSCCD)},
  author={Vielhaben, Johanna and Bl{\"u}cher, Stefan and Strodthoff, Nils},
  journal={arXiv preprint arXiv:2203.06043},
  year={2022}
}

@inproceedings{zhang2021learning,
  title={Learning a self-expressive network for subspace clustering},
  author={Zhang, Shangzhi and You, Chong and Vidal, Ren{\'e} and Li, Chun-Guang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12393--12403},
  year={2021}
}

@article{kang2021structured,
  title={Structured graph learning for scalable subspace clustering: From single view to multiview},
  author={Kang, Zhao and Lin, Zhiping and Zhu, Xiaofeng and Xu, Wenbo},
  journal={IEEE Transactions on Cybernetics},
  year={2021},
  publisher={IEEE}
}

@inproceedings{samaria1994parameterisation,
  title={Parameterisation of a stochastic model for human face identification},
  author={Samaria, Ferdinando S and Harter, Andy C},
  booktitle={Proceedings of 1994 IEEE workshop on applications of computer vision},
  pages={138--142},
  year={1994},
  organization={IEEE}
}

@article{von2007tutorial,
  title={A tutorial on spectral clustering},
  author={Von Luxburg, Ulrike},
  journal={Statistics and computing},
  volume={17},
  number={4},
  pages={395--416},
  year={2007},
  publisher={Springer}
}

@article{donoho2006most,
  title={For most large underdetermined systems of linear equations the minimal ��1-norm solution is also the sparsest solution},
  author={Donoho, David L},
  journal={Communications on Pure and Applied Mathematics: A Journal Issued by the Courant Institute of Mathematical Sciences},
  volume={59},
  number={6},
  pages={797--829},
  year={2006},
  publisher={Wiley Online Library}
}

@article{candes2005decoding,
  title={Decoding by linear programming},
  author={Candes, Emmanuel J and Tao, Terence},
  journal={IEEE transactions on information theory},
  volume={51},
  number={12},
  pages={4203--4215},
  year={2005},
  publisher={IEEE}
}

@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society: Series B (Methodological)},
  volume={58},
  number={1},
  pages={267--288},
  year={1996},
  publisher={Wiley Online Library}
}

@article{ng2001spectral,
  title={On spectral clustering: Analysis and an algorithm},
  author={Ng, Andrew and Jordan, Michael and Weiss, Yair},
  journal={Advances in neural information processing systems},
  volume={14},
  year={2001}
}

@article{liu2021self,
  title={Self-Supervised Convolutional Subspace Clustering Network with the Block Diagonal Regularizer},
  author={Liu, Maoshan and Wang, Yan and Ji, Zhicheng},
  journal={Neural Processing Letters},
  volume={53},
  number={6},
  pages={3849--3875},
  year={2021},
  publisher={Springer}
}

@inproceedings{zhu2021self,
  title={Self-Supervised Embedding for Subspace Clustering},
  author={Zhu, Wenjie and Peng, Bo and Chen, Chunchun},
  booktitle={Proceedings of the 30th ACM International Conference on Information \& Knowledge Management},
  pages={3687--3691},
  year={2021}
}

@inproceedings{wang2018co,
  title={Co-referenced subspace clustering},
  author={Wang, Xiaobo and Lei, Zhen and Shi, Hailin and Guo, Xiaojie and Zhu, Xiangyu and Li, Stan Z},
  booktitle={2018 IEEE International Conference on Multimedia and Expo (ICME)},
  pages={1--6},
  year={2018},
  organization={IEEE}
}

@article{chandra2020forecasting,
  title={Forecasting trajectory and behavior of road-agents using spectral clustering in graph-lstms},
  author={Chandra, Rohan and Guan, Tianrui and Panuganti, Srujan and Mittal, Trisha and Bhattacharya, Uttaran and Bera, Aniket and Manocha, Dinesh},
  journal={IEEE Robotics and Automation Letters},
  volume={5},
  number={3},
  pages={4882--4890},
  year={2020},
  publisher={IEEE}
}

@article{zhao2019fast,
  title={Fast spectral clustering for unsupervised hyperspectral image classification},
  author={Zhao, Yang and Yuan, Yuan and Wang, Qi},
  journal={Remote Sensing},
  volume={11},
  number={4},
  pages={399},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@article{janani2019text,
  title={Text document clustering using spectral clustering algorithm with particle swarm optimization},
  author={Janani, R and Vijayarani, S},
  journal={Expert Systems with Applications},
  volume={134},
  pages={192--200},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{liu2013large,
  title={Large-scale spectral clustering on graphs},
  author={Liu, Jialu and Wang, Chi and Danilevsky, Marina and Han, Jiawei},
  booktitle={Twenty-Third International Joint Conference on Artificial Intelligence},
  year={2013},
  organization={Citeseer}
}

@article{ding2012two,
  title={Two-step spectral clustering controlled islanding algorithm},
  author={Ding, Lei and Gonzalez-Longatt, Francisco M and Wall, Peter and Terzija, Vladimir},
  journal={IEEE Transactions on Power Systems},
  volume={28},
  number={1},
  pages={75--84},
  year={2012},
  publisher={IEEE}
}

@inproceedings{song2008parallel,
  title={Parallel spectral clustering},
  author={Song, Yangqiu and Chen, Wen-Yen and Bai, Hongjie and Lin, Chih-Jen and Chang, Edward Y},
  booktitle={Joint European conference on machine learning and knowledge discovery in databases},
  pages={374--389},
  year={2008},
  organization={Springer}
}

@article{huang2019ultra,
  title={Ultra-scalable spectral clustering and ensemble clustering},
  author={Huang, Dong and Wang, Chang-Dong and Wu, Jian-Sheng and Lai, Jian-Huang and Kwoh, Chee-Keong},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={32},
  number={6},
  pages={1212--1226},
  year={2019},
  publisher={IEEE}
}

@inproceedings{peng2013scalable,
  title={Scalable sparse subspace clustering},
  author={Peng, Xi and Zhang, Lei and Yi, Zhang},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={430--437},
  year={2013}
}


@inproceedings{li2011time,
  title={Time and space efficient spectral clustering via column sampling},
  author={Li, Mu and Lian, Xiao-Chen and Kwok, James T and Lu, Bao-Liang},
  booktitle={CVPR 2011},
  pages={2297--2304},
  year={2011},
  organization={IEEE}
}

@inproceedings{kong2011fast,
  title={A fast incremental spectral clustering for large data sets},
  author={Kong, Tengteng and Tian, Ye and Shen, Hong},
  booktitle={2011 12th International Conference on Parallel and Distributed Computing, Applications and Technologies},
  pages={1--5},
  year={2011},
  organization={IEEE}
}

@inproceedings{li2016scalable,
  title={Scalable sequential spectral clustering},
  author={Li, Yeqing and Huang, Junzhou and Liu, Wei},
  booktitle={Thirtieth AAAI conference on artificial intelligence},
  year={2016}
}

@article{langone2017fast,
  title={Fast kernel spectral clustering},
  author={Langone, Rocco and Suykens, Johan AK},
  journal={Neurocomputing},
  volume={268},
  pages={27--33},
  year={2017},
  publisher={Elsevier}
}

@article{he2018fast,
  title={Fast large-scale spectral clustering via explicit feature mapping},
  author={He, Li and Ray, Nilanjan and Guan, Yisheng and Zhang, Hong},
  journal={IEEE transactions on cybernetics},
  volume={49},
  number={3},
  pages={1058--1071},
  year={2018},
  publisher={IEEE}
}

@article{zhang2019robust,
  title={Robust low-rank kernel multi-view subspace clustering based on the schatten p-norm and correntropy},
  author={Zhang, Xiaoqian and Sun, Huaijiang and Liu, Zhigui and Ren, Zhenwen and Cui, Qiongjie and Li, Yanmeng},
  journal={Information Sciences},
  volume={477},
  pages={430--447},
  year={2019},
  publisher={Elsevier}
}

@article{zhu2020sparse,
  title={Sparse and low-rank regularized deep subspace clustering},
  author={Zhu, Wenjie and Peng, Bo},
  journal={Knowledge-Based Systems},
  volume={204},
  pages={106199},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{hefeeda2012distributed,
  title={Distributed approximate spectral clustering for large-scale datasets},
  author={Hefeeda, Mohamed and Gao, Fei and Abd-Almageed, Wael},
  booktitle={Proceedings of the 21st international symposium on High-Performance Parallel and Distributed Computing},
  pages={223--234},
  year={2012}
}


@article{wu2019essential,
  title={Essential tensor learning for multi-view spectral clustering},
  author={Wu, Jianlong and Lin, Zhouchen and Zha, Hongbin},
  journal={IEEE Transactions on Image Processing},
  volume={28},
  number={12},
  pages={5910--5922},
  year={2019},
  publisher={IEEE}
}

@inproceedings{bianchi2020spectral,
  title={Spectral clustering with graph neural networks for graph pooling},
  author={Bianchi, Filippo Maria and Grattarola, Daniele and Alippi, Cesare},
  booktitle={International Conference on Machine Learning},
  pages={874--883},
  year={2020},
  organization={PMLR}
}

@article{zhu2018one,
  title={One-step multi-view spectral clustering},
  author={Zhu, Xiaofeng and Zhang, Shichao and He, Wei and Hu, Rongyao and Lei, Cong and Zhu, Pengfei},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={31},
  number={10},
  pages={2022--2034},
  year={2018},
  publisher={IEEE}
}

@inproceedings{huang2019multi,
  title={Multi-view Spectral Clustering Network.},
  author={Huang, Zhenyu and Zhou, Joey Tianyi and Peng, Xi and Zhang, Changqing and Zhu, Hongyuan and Lv, Jiancheng},
  booktitle={IJCAI},
  pages={2563--2569},
  year={2019}
}

@article{kang2020multi,
  title={Multi-graph fusion for multi-view spectral clustering},
  author={Kang, Zhao and Shi, Guoxin and Huang, Shudong and Chen, Wenyu and Pu, Xiaorong and Zhou, Joey Tianyi and Xu, Zenglin},
  journal={Knowledge-Based Systems},
  volume={189},
  pages={105102},
  year={2020},
  publisher={Elsevier}
}


@inproceedings{abavisani2018adversarial,
  title={Adversarial domain adaptive subspace clustering},
  author={Abavisani, Mahdi and Patel, Vishal M},
  booktitle={2018 IEEE 4th International Conference on Identity, Security, and Behavior Analysis (ISBA)},
  pages={1--8},
  year={2018},
  organization={IEEE}
}

@article{abavisani2018multimodal,
  title={Multimodal sparse and low-rank subspace clustering},
  author={Abavisani, Mahdi and Patel, Vishal M},
  journal={Information Fusion},
  volume={39},
  pages={168--177},
  year={2018},
  publisher={Elsevier}
}

@article{zhu2019multi,
  title={Multi-view deep subspace clustering networks},
  author={Zhu, Pengfei and Hui, Binyuan and Zhang, Changqing and Du, Dawei and Wen, Longyin and Hu, Qinghua},
  journal={arXiv preprint arXiv:1908.01978},
  year={2019}
}

@inproceedings{sun2019self,
  title={Self-supervised deep multi-view subspace clustering},
  author={Sun, Xiukun and Cheng, Miaomiao and Min, Chen and Jing, Liping},
  booktitle={Asian Conference on Machine Learning},
  pages={1001--1016},
  year={2019},
  organization={PMLR}
}

@article{peng2016constructing,
  title={Constructing the L2-graph for robust subspace learning and subspace clustering},
  author={Peng, Xi and Yu, Zhiding and Yi, Zhang and Tang, Huajin},
  journal={IEEE transactions on cybernetics},
  volume={47},
  number={4},
  pages={1053--1066},
  year={2016},
  publisher={IEEE}
}

@article{cai2020graph,
  title={Graph convolutional subspace clustering: A robust subspace clustering framework for hyperspectral image},
  author={Cai, Yaoming and Zhang, Zijia and Cai, Zhihua and Liu, Xiaobo and Jiang, Xinwei and Yan, Qin},
  journal={IEEE Transactions on Geoscience and Remote Sensing},
  volume={59},
  number={5},
  pages={4191--4202},
  year={2020},
  publisher={IEEE}
}

@article{wang2021multi,
  title={Multi-scale graph attention subspace clustering network},
  author={Wang, Tong and Wu, Junhua and Zhang, Zhenquan and Zhou, Wen and Chen, Guang and Liu, Shasha},
  journal={Neurocomputing},
  volume={459},
  pages={302--314},
  year={2021},
  publisher={Elsevier}
}

@article{xu2019scaled,
  title={Scaled simplex representation for subspace clustering},
  author={Xu, Jun and Yu, Mengyang and Shao, Ling and Zuo, Wangmeng and Meng, Deyu and Zhang, Lei and Zhang, David},
  journal={IEEE Transactions on Cybernetics},
  volume={51},
  number={3},
  pages={1493--1505},
  year={2019},
  publisher={IEEE}
}

@article{stallkamp2012man,
  title={Man vs. computer: Benchmarking machine learning algorithms for traffic sign recognition},
  author={Stallkamp, Johannes and Schlipsing, Marc and Salmen, Jan and Igel, Christian},
  journal={Neural networks},
  volume={32},
  pages={323--332},
  year={2012},
  publisher={Elsevier}
}

@article{abdolali2021beyond,
  title={Beyond linear subspace clustering: A comparative study of nonlinear manifold clustering algorithms},
  author={Abdolali, Maryam and Gillis, Nicolas},
  journal={Computer Science Review},
  volume={42},
  pages={100435},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{wang2010locality,
  title={Locality-constrained linear coding for image classification},
  author={Wang, Jinjun and Yang, Jianchao and Yu, Kai and Lv, Fengjun and Huang, Thomas and Gong, Yihong},
  booktitle={2010 IEEE computer society conference on computer vision and pattern recognition},
  pages={3360--3367},
  year={2010},
  organization={IEEE}
}

@article{roweis2000nonlinear,
  title={Nonlinear dimensionality reduction by locally linear embedding},
  author={Roweis, Sam T and Saul, Lawrence K},
  journal={science},
  volume={290},
  number={5500},
  pages={2323--2326},
  year={2000},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{cai2022efficient,
  title={Efficient Deep Embedded Subspace Clustering},
  author={Cai, Jinyu and Fan, Jicong and Guo, Wenzhong and Wang, Shiping and Zhang, Yunhe and Zhang, Zhao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1--10},
  year={2022}
}


